Disentangled Relational Representations for Explaining and Learning from Demonstration

Learning from demonstration is an effective method for human users to instruct desired robot behaviour. However, for most non-trivial tasks of practical interest, efficient learning from demonstration depends crucially on inductive bias in the chosen structure for rewards/costs and policies. We address the case where this inductive bias comes from an exchange with a human user. We propose a method in which a learning agent utilizes the information bottleneck layer of a high-parameter variational neural model, with auxiliary loss terms, in order to ground abstract concepts such as spatial relations. The concepts are referred to in natural language instructions and are manifested in the high-dimensional sensory input stream the agent receives from the world. We evaluate the properties of the latent space of the learned model in a photorealistic synthetic environment and particularly focus on examining its usability for downstream tasks. Additionally, through a series of controlled table-top manipulation experiments, we demonstrate that the learned manifold can be used to ground demonstrations as symbolic plans, which can then be executed on a PR2 robot.

==> content/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
Through the performed ablation study we can see that the model which incorporates both a reconstruction loss term and a Softmax cross-entropy term performs best when it comes down to identifying the movement prescription sequences in the repetitive movement demonstrations. This supports our hypothesis that by object label classification and by utilising the full dataset through the reconstruction loss, we learn smoother and more factorised vectors $\mathbf{z}$ and $\mathbf{c}$ which allows for the task segmentation process to be more efficient. Notably the same model under-performs on the last concept group---out/in. We hypothesize that might be caused due to the bigger imbalance in labelled/unlabelled data pairs as compared to the other concept groups. As far as the chained movement demonstrations are concerned, all models perform in an equal manner, which is expected, since these sequences only involve a single object moving.
The best performing model from Table \ref{table:plan_segmentation_acc} (a) is used on the symbolic plan inference task over the demonstrated chained behaviour (where the underlying plan is over a single target object and is a multi-step one). Figure \ref{fig:rel_chaining_ed} reports the average edit distance for the plans inferred over all demonstrations for a given task (top row). Additionally, the average plan lengths is also reported. Both quantities are reported as a function of the number of demonstrations used to infer the task essence which in turn is used to infer the step-by-step plan for each demonstration. As expected, the more demonstration we see, the closer the inferred plans get to the ground truth ones, both in terms of lengths and meaning. The reason why some of the plots do not converge to the ground-truth numbers (red line across all plots in the figure) can be assignment to the fact that some demonstrations contain occlusions between the objects, making them hard to reliably infer the true plan without noise.
Lastly, Figure \ref{fig:res_all_robot_eef_mae} reports the mean absolute error across all axis for the three demonstrated tasks. What is reflected in the plots is the fact that for certain tasks the model learn to predict more reliably only along the end effector axes that matter for the success of the task---e.g. for placing \textit{on} and \textit{in} we get lower error across X/Y/Z as compared to when making the cups \textit{face} each other. Respectively, the \textit{facing} tasks puts more weight on the Roll and Pitch axes (which matter for the cups to have the right orientation) and not so much weight on the Yaw axis or on the translational X/Y/Z. 
